SEINE: SEgment-based Indexing for NEural information retrieval

Many early neural Information Retrieval (NeurIR) methods are re-rankers that rely on a traditional first-stage retriever due to expensive query time computations. Recently, representation-based retrievers have gained much attention, which learns query representation and document representation separately, making it possible to pre-compute document representations offline and reduce the workload at query time. Both dense and sparse representation-based retrievers have been explored. However, these methods focus on finding the representation that best represents a text (aka metric learning) and the actual retrieval function that is responsible for similarity matching between query and document is kept at a minimum by using dot product. One drawback is that unlike traditional term-level inverted index, the index formed by these embeddings cannot be easily re-used by another retrieval method. Another drawback is that keeping the interaction at minimum hurts retrieval effectiveness. On the contrary, interaction-based retrievers are known for their better retrieval effectiveness. In this paper, we propose a novel SEgment-based Neural Indexing method, SEINE, which provides a general indexing framework that can flexibly support a variety of interaction-based neural retrieval methods. We emphasize on a careful decomposition of common components in existing neural retrieval methods and propose to use segment-level inverted index to store the atomic query-document interaction values. Experiments on LETOR MQ2007 and MQ2008 datasets show that our indexing method can accelerate multiple neural retrieval methods up to 28-times faster without sacrificing much effectiveness.

==> abstract.tex <==


Neural Information Retrieval (NeurIR) methods have achieved top performance for ad hoc retrieval. Most neural retrieval methods, however, are re-ranking models that rely on traditional retrieval methods for first-stage retrieval. Re-ranking is necessary because these models must process each document at query time using computationally expensive neural networks. In this paper, we propose a novel SEgment-based Neural Indexing method, SEINE, that moves heavy computations offline and only keeps essential calculations at query time. Our method is a modern version of the classic split of ad hoc retrieval into indexing and retrieval phases. In addition, we propose a flexible segment-based indexing approach to support neural retrieval methods that perform query-document interaction at different granularities. Experiments on LETOR MQ2007 and MQ2008 datasets show that our index can make neural retrieval methods up to 28-times faster without sacrificing much effectiveness. 



% Our VBNI can also support passage retrieval tasks. The results on Squad 2.0 dataset demonstrate that ... 


%because of the high inefficiency in processing documents and producing interaction matrix in real-time retrieval. This inefficiency makes the NeurIR models rely on first-stage retrieval models, such as BM25, and hard to use as commercial web search engines.

% a Visualization-Based Neural Indexing (VBNI) method to support NeurIR models.  We first build vocabulary for the entire corpus by filtering out stopwords. Then we do term-document interaction of the vocabulary and corpus by frequency-based and vector-based features. Finally, these interactions are stored in an Inverted Index for further retrieval tasks.

==> exp_qa.tex <==
\section{Experiments on Passage Retrieval Task for QA}
Common passage retrieval models \cite{yang2019end} \cite{izacard2020leveraging} contains two steps:
1) Passage retrieval: They first split the documents into fixed length segments. Then for each query, top-K segments are retrieved using traditional inverted index and BM25.
2) Answer selection: The query and top-K segments are fed into a deep neural network such as BERT \cite{devlin2018bert}, the answer span is finally learned.

In this section, we conduct experiments using Neu-IR models with our index to do passage retrieval on SQuAD v1.1 dataset. 
It demonstrates our index can be applied other IR tasks such as passage retrieval for QA. 

\subsection{Dataset and Metrics}
We conduct our experiments on Stanford Question Answering Dataset (SQuAD) v1.1, a reading comprehension dataset consisting of 100,000+ questions on a set of Wikipedia articles \cite{rajpurkar2016squad}.
The collection we used is the Wikipedia corpus (from Dec. 2016; containing 5 million articles).
Following Chen et al. \cite{chen2017reading}, we use exact match (EM) score and F1 score (at the token level) as the evaluation metrics.

\subsection{Baselines}
We choose three Neu-IR models and two Neural Indexing models as our baselines for comparison:
\begin{itemize}
    \item BM25 with traditional inverted index.
    \item DeepTileBars with our index. 
\end{itemize}

\subsection{Answer Selection with BERTserini}
We use BERTserini \cite{yang2019end} as the answer selection method. 
After top-K segments are retrieved given a query, the query and segments together are fed as input into BERT model to get the answer span. 
The parameters are all set default following Yang et. al paper.

\subsection{Results}



==> oldtable.tex <==
\begin{table*}[htb]
\footnotesize
\caption{Retrieval Effectiveness and Efficiency on MQ2007 and MQ2008. %Improvement (percentage for effectiveness and times for efficiency) of each metric is obtained by comparing to corresponding retrieval method with No Index. 
$^*$ denotes statistically significant degradation on effectiveness and $^\dagger$ for statistically significant improvement on efficiency compared to corresponding retrieval method with ``No Index".}  \sibo{I think we can change "DeepCT" to "DeepCT-bm25", which indicate using DeepCT weight to do BM25, then it will be a retrieval method and move under SEINE indexing. } \grace{fine. But make sure you write sufficient and clear descriptions in the main text (probably at multiple places) to explain. Do not just write one sentence without sufficient argumentation, reasoning and citations.} 
\label{tab:result} 
\subtable[\textbf{MQ2007.}]{
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{2}{l}*{5}{lr}*{4}{r}}
\toprule
    \multirow{3}{*}{\bf Indexing} &  \multirow{3}{*}{\bf Retrieval}  &  \multicolumn{10}{c}{\bf Effectiveness}  &  \multicolumn{4}{c}{\bf Efficiency}\\ 
\cline{3-12} \cline{13-16} 
    &  & \multicolumn{2}{c}{P@5}  & \multicolumn{2}{c}{P@10}  & \multicolumn{2}{c}{MAP} & \multicolumn{2}{c}{nDCG@5} & \multicolumn{2}{c}{nDCG@10}  & \multicolumn{2}{c}{Training (ms)} & \multicolumn{2}{c}{Test (ms)} \\
\cline{2-4} \cline{5-6} \cline{7-8} \cline{9-10} \cline{11-12} \cline{13-14} \cline{15-16}       
No Index& Dot Product &0.328&&0.344&&0.418&&0.282&&0.332& &&&& \\
        & KNRM  &0.355&&0.382&&0.461&&0.379&&0.412&&42.63&&16.70& \\ 
        & HiNT$\diamond$  &0.461&&0.418&&0.505&&0.463&&0.490&&1139.34&&1009.11& \\
        & DeepTileBars  &0.429&&0.408&&0.474&&0.398&&0.434&&163.91&&73.68& \\
\cline{2-16}
InvIdx$^\ddagger$& BM25$\diamond$    &0.388&&0.366&&0.456&&0.384&&0.414&&&&& \\
        % & KNRM    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
        % & HiNT    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
        % & DeepTileBars    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
\cline{2-16}
DeepCT$^\ddagger$ & BM25    &0.315&&0.327&&0.397&&0.266&&0.314&&&&&  \\
        % & KNRM    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
        % & HiNT    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
        % & DeepTileBars    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
\cline{2-16}
SNRM    & Dot Product   &0.288$^*$&-12\%&0.307$^*$&-11\%&0.368$^*$&-10\%&0.254$^*$&-9\%&0.302$^*$&-9\%&&&& \\
        & KNRM  &0.322$^*$&-9\%&0.347$^*$&-9\% &0.417$^*$&-10\%&0.337$^*$&-11\%&0.404&-2\%
                &35.56&1.2$\times$&13.17&1.3$\times$\\
        & HiNT  &0.401$^*$&-13\%&0.358$^*$&-14\%&0.423$^*$&-16\%&0.379$^*$&-18\%&0.402$^*$&-18\%
                &958.03&1.2$\times$&860.76&1.1$\times$ \\
        & DeepTileBars  &0.281$^*$&-35\%&0.304$^*$&-25\%&0.359$^*$&-24\%&0.238$^*$&-40\%&0.290$^*$&-33\%
                        & 131.43 & 1.2$\times$ & 56.97& 1.3$\times$ \\
\cline{2-16}   
SEINE    & Dot Product &0.328&0\%&0.344&0\%&0.418&0\%&0.282&0\%&0.332&0\%&&&&\\
        & KNRM  &0.342&-4\%&0.372&-2\%&0.447&-3\%&0.374&-1\%&0.401&-3\%
                &11.67$^\dagger$&3.7$\times$&1.22$^\dagger$&13.7$\times$ \\
        & HiNT  &0.453&-2\%&0.409&-2\%&0.492&-3\%&0.452&-2\%&0.483&-3\%
                &834.64&1.4$\times$&706.42&1.4$\times$ \\ 
        & DeepTileBars  &0.412&-4\%&0.404&-1\%&0.468&-1\%&0.391&-2\%&0.427&-2\%         &22.62$^\dagger$&7.4$\times$&2.67$^\dagger$&28.1$\times$ \\
\bottomrule
\end{tabular*}
} 
%\vspace{-0.07in} 
\subtable[\textbf{MQ2008.}]{ 
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{2}{l}*{5}{lr}*{4}{r}}
\toprule
    \multirow{3}{*}{\bf Indexing} &  \multirow{3}{*}{\bf Retrieval}  &  \multicolumn{10}{c}{\bf Effectiveness}  &  \multicolumn{4}{c}{\bf Efficiency}\\ 
\cline{3-12} \cline{13-16} 
    &  & \multicolumn{2}{c}{P@5}  & \multicolumn{2}{c}{P@10}  & \multicolumn{2}{c}{MAP} & \multicolumn{2}{c}{nDCG@5} & \multicolumn{2}{c}{nDCG@10}  & \multicolumn{2}{c}{Training (ms)} & \multicolumn{2}{c}{Test (ms)} \\
\cline{2-4} \cline{5-6} \cline{7-8} \cline{9-10} \cline{11-12} \cline{13-14} \cline{15-16} 
No Index& Dot Product   &0.333&&0.281&&0.462&&0.411&&0.183&&&&&\\
        & KNRM  &0.355&&0.355&&0.472&&0.499&&0.225&
                &41.27&&16.86&\\
        & HiNT$\diamond$  &0.367&&0.255&&0.505&&0.501&&0.244&     
                &1139.34&&1009.11&\\
        & DeepTileBars  &0.425&&0.321&&0.567&&0.548&&0.259&
                        &167.20&&74.96& \\
\cline{2-16}
InvIdx$^\ddagger$  & BM25$\diamond$  &0.337&&0.245&&0.465&&0.461&&0.220&&& \\
        % & KNRM  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
        % & HiNT  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
        % & DeepTileBars  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
\cline{2-16}
DeepCT$^\ddagger$  & BM25  &0.307&&0.239&&0.448&&0.400&&0.197&&&&&  \\
        % & KNRM  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
        % & HiNT  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
        % & DeepTileBars  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
\cline{2-16}
SNRM    & Dot Product  &0.380$^\dagger$&14\%&0.300$^\dagger$&7\%&0.513$^\dagger$&11\%&0.483$^\dagger$&18\%&0.223$^\dagger$&22\%&&&& \\
        & KNRM  &0.303$^*$&-15\%&0.229$^*$&-10\%&0.417$^*$&-12\%&0.417$^*$&-16\%&0.199$^*$&-12\%
                &36.78&1.1$\times$&12.68&1.3$\times$ \\
        & HiNT  &0.291$^*$&-21\%&0.209$^*$&-18\%&0.401$^*$&-21\%&0.445$^*$&-11\%&0.221$^*$&-10\%
                &941.09&1.2$\times$&904.16&1.1$\times$\\
        & DeepTileBars  &0.356$^*$&-16\%&0.291$^*$&-9\%&0.481$^*$&-15\%&0.434$^*$&-21\%&0.200$^*$&-23\% 
                        &134.10&1.2$\times$&58.14&1.3$\times$ \\
\cline{2-16}
SEINE    & Dot Product   &0.333&0\%&0.281&0\%&0.462&0\%&0.411&0\%&0.183&0\%&&&& \\
        & KNRM  &0.346&-3\%&0.252&-1\%&0.462&-2\%&0.485&-3\%&0.218&-3\%  
                &11.58$^\dagger$&3.6$\times$&1.24$^\dagger$&13.6$\times$ \\
        & HiNT  &0.362&-1\%&0.250&-2\%&0.485&-4\%&0.489&-2\%&0.236&-3\%
                &828.84&1.4$\times$&687.85&1.5$\times$ \\ 
        & DeepTileBars &0.422&-1\%&0.322&0\%&0.569&0\%&0.544&-1\%&0.255&-2\%
             &22.62$^\dagger$&7.4$\times$&2.67$^\dagger$&28.1$\times$ \\
\bottomrule
\end{tabular*}
}
\leftline{\tabnote{$^\diamond$ Results reported in Fan et al. \cite{fan2018modeling}. $^\ddagger$ Indexing method is not applicable to KNRM, HiNT, and DeepTileBars.} }
\end{table*} 

==> oldtext.tex <==


(2) Even if we do not decompose the transformer blocks of all-in-all interactions, it is still impossible to store the q-d interaction in the index. We assume the vocabulary contains all the query terms when doing term-level interaction. The vocabulary terms can be decided by the document corpus. However, there is no such "vocabulary" containing all the queries. 
Therefore, the limitations of our index design make us can only focus on sparse, interaction-based methods.
\sibo{end} 

====

% We have examined most popular non-transformer NeurIR methods, and design the following features to keep in an inverted index to support most of them.  Our features focus on interaction between a term and an interaction unit, which can be a document, term, or segment. The features include  term frequency, inverse document frequency, semantic neighboring, dot product and cosine similarity. For each term $w$ and an interaction unit $S$, we pre-calculate and store the following feature values:  

%\grace{sibo, please edit this part to be flexible, general,  and include deepct weight and tilde pr(t|d). Also write nice text descriptions to explain. } 
% \begin{equation}
% \label{eq:mat} \small
% M(w, S)=\left\{  
% \begin{array}{l} 
%     tf(w, S) \times idf(w) \times \mathbb I_S(w) \qquad frequency-based\\
%     \sum_{t \in S} E(w) \cdot E(t) \qquad\qquad similarity\\
%     \max_{t \in S} exp(-(E(w)-E(t))^2) \qquad\qquad kernel\ function\\
%     \sum_{t \in S} a\cdot E_t(S) + b \qquad\qquad linear\ function \\
%     \sum_{t \in S} P_\theta(E(w) | E(S)) \qquad\qquad log\ probability
%     %\sum_{t \in S} cos(v_w, v_t)\\
% \end{array} 
% \right.  
% \end{equation} 
% where $tf(w, S)$ is the term frequency of $w$ in $S$, $idf(w)$ is the inverse document frequency of $w$. 
% $\mathbb I_S(w)$ is the indicator function showing whether $w$ is in $S$.
% Word vectors $v_w$ and $v_t$ are embeddings from a pre-trained word2vec model \cite{mikolov2013distributed}, which are used to calculate the between-word similarity. $\max_{t \in S} e^{-(v_{w}-v_t)^2}$ is a kernel function proposed by \cite{xiong2017end} to measure semantic neighborhood. Similarly, dot product and cosine similarity $cos(\cdot, \cdot)$ are also common measures to evaluate similarity between two term vectors.
% These features tf, idf, and word similarity measures are all proven to be essential for ad-hoc retrieval and widely used in NeuIR models. One can choose a subset of features or update this feature list.

 
%\grace{Note we have used v-d interactions (and some places are v-S interactions. Please edit the following (and the rest of the paper) accordingly. } 



======


% One solution is to move heavy computations in a NeurIR method to offline and only keeps essential calculations at query time. The idea follows the classic split of the entire ad hoc retrieval pipeline into indexing and retrieval phases. Traditional IR systems use an inverted index, which is computed offline and stores the term frequency (tf) of each term in each document at the indexing phase. Although it may take a long time to build the index, the pre-computed term frequency scores can be directly retrieved from the index and used at the retrieval phase, making the retrieval time much shorter. Unlike conventional IR methods, NeurIR models do not have an index; therefore, they cannot save the query-time computations by doing part of them offline, and can only work with smaller datasets. 


=======

SEINE applies to different NeurIR methods by simply modifying the unit of text for interaction. 


In addition, we do not face SNRM's vocabulary mismatch problem. ~\justin{earlier in the text, we mentioned that we might face a vocab mismatch problem because we assume that all query terms are in the corpus. I don't think this is relevant here, but reviewers might be confused by our earlier comment} \grace{I think we both have the issue. Need Sibo's input} \sibo{1) out-of-vocabulary problem, is that a new query term may not in the vocabulary, but we assume that all query terms are in the corpus as many IR methods; 2) the mismatch problem is SNRM is that they generate new latent terms which has a larger possibility it's not in the index. My idea is remove this sentence: "In addition ... mismatch problem."} 


========

% The segmentation is done based on lexical co-occurrence and distribution, aiming to better reflect the discourse structure in a document than fixed-size window segmentation. 

\justin{start edit} 
After computing the similarity between all windows of text in the document, it splits the document into topical segments where two adjacent windows have the lowest similarity scores. ~\justin{end edit}

==========

% we calculate and store the interaction matrices for each term in the vocabulary and each document in an index.



% We first build a vocabulary for the entire corpus by filtering out stopwords and performing word normalization. Second, we use TextTiling \cite{hearst1994multi} to split documents into topical segments. 
% Third, we calculate the segment-level interaction for each term in the vocabulary and each document in the corpus by features supporting exact matching, including term frequency (tf), inverse document frequency (idf), and features supporting semantic matching that focus on  calculating similarities between words \cite{mitchell2010composition}, including semantic neighboring, dot product and cosine similarity \cite{boytsov2016off}. 
% Fourth, these features are stored in the inverted index for further retrieval tasks. Using this inverted index, SEINE departs from the re-ranking paradigm, allowing for end-to-end retrieval. 


=======


%In contrast to the majority of existing neural methods, our index is designed to be query-independent. 
%Based on the assumption that all query terms are in the vocabulary of the document corpus, 


==========

\begin{comment}
\begin{table*}
  \caption{Results on QA dataset.}
  \label{tab:qa}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{12}{l}}
    \toprule
    \multirow{4}{*}{\bf Indexing} &  \multirow{4}{*}{\bf Retrieval}  &  \multicolumn{6}{c}{\bf Effectiveness}  &  \multicolumn{4}{c}{\bf Efficiency}\\ 
    \cline{3-8} \cline{9-12} \\
    &  & \multicolumn{2}{c}{P@5}  & \multicolumn{2}{c}{MAP}  & \multicolumn{2}{c}{NDCG@5} & \multicolumn{2}{c}{Training (ms)} & \multicolumn{2}{c}{Test (ms)} \\
    \cline{3-4} \cline{5-6} \cline{7-8} \cline{9-10} \cline{11-12} \\ 
    InvIdx  
         & BM25         &&&&&&&&&& \\
         & DeepTileBars &&&&&&&&&& \\
    \cline{2-12}    
    SEINE 
         & Dot Product  &&&&&&&&&& \\
         & DeepTileBars &&&&&&&&&& \\
    \bottomrule
\end{tabular*}
\end{table*}
\end{comment}

\begin{comment}
\begin{table*}
%\small
\footnotesize
  \caption{Results on MQ2008. 
  Improvement (percentage for effectiveness and times for efficiency) of each metrics is comparing to the corresponding retrieval method + No index. 
  $^*$ indicates statistically significant improvements over SNRM + DotProduct. Non-applicable cells filled with `--'.} 
  %\grace{1)use cite; dont hard code citation. 2) add one more col for each metric, so that each metric has its own value and the Impr. (improvement). 3) remove some metrics due to space issue. The table needs to be shown within text width. 4) fill up non-applicable cells with `--' }
  \label{tab:mq08}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{2}{l}*{6}{lr}*{4}{r}}
    %\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{12}{l}}
    \toprule
    \multirow{4}{*}{\bf Retrieval} &  \multirow{4}{*}{\bf Indexing}  &  \multicolumn{12}{c}{\bf Effectiveness}  &  \multicolumn{4}{c}{\bf Efficiency}\\ 
    \cline{3-14} \cline{15-18} \\
    &  & \multicolumn{2}{c}{P@5}  & \multicolumn{2}{c}{P@10}  & \multicolumn{2}{c}{MAP} & \multicolumn{2}{c}{NDCG@5} & \multicolumn{2}{c}{NDCG@10}  & \multicolumn{2}{c}{Mean NDCG} & \multicolumn{2}{c}{Training (ms)} & \multicolumn{2}{c}{Test (ms)} \\
    \cline{3-4} \cline{5-6} \cline{7-8} \cline{9-10} \cline{11-12} \cline{13-14} \cline{15-16} \cline{17-18} \\ 
    BM25        & InvIdx    & 0.337 &--& 0.245 &--& 0.465 &--& 0.461 &--& 0.220 &-- &--&--&--&-- \\
                & DeepCT    &&--&&--&&--&&-- &--&--&--&--  \\
    Dot Product & SNRM      & 0.380 &--& 0.300 &--& 0.513 &--& 0.483 &--& 0.223 &-- &--&--&--&-- \\
    \cline{2-18}
    KNRM    & No Index  & 0.364 && 0.250 && 0.474 && 0.494 && 0.237 &  &0.xxx&-xx\%      
                        & 41.27 && 16.86 & \\
            & InvIdx    &--&--&--&--&--&--&--&--&--&--&--&--&--&--   \\
            & DeepCT    &--&--&--&--&--&--&--&--&--&--&--&--&--&--   \\
            & SNRM      & 0.297 & -14\% & 0.196 & -22\% & 0.377 & -21\% & 0.393 & -21\% & 0.199 & -16\% &0.xxx&-xx\% 
                        & 36.78 & 4.6$\times$ & 12.68 & 5.5$\times$ \\
            & SEINE      & 0.339 & -2\% & 0.245 & -2\% & 0.466 & -2\% & 0.467 & -4\% & 0.231 & -2\%  &0.xxx&-xx\%  
                        & 11.58 & 13.9$\times$ & 1.24 & 59.3$\times$ \\
    \cline{2-18}
    HiNT    & No Index  & 0.367 && 0.255 && 0.505 && 0.501 && 0.244 & &0.xxx&-xx\%     
                        & 1139.34 & & 1009.11 & \\
            & InvIdx    &--&--&--&--&--&--&--&--&--&--&--&--&--&--   \\
            & DeepCT    &--&--&--&--&--&--&--&--&--&--&--&--&--&--   \\
            & SNRM      & 0.300 & -18\% & 0.224 & -12\% & 0.456 & -10\% & 0.412 & -18\% & 0.192 & -21\% &0.xxx&-xx\% 
                        &&&& \\
            & SEINE      & 0.354 & -4\% & 0.247 & -3\% & 0.495 & -2\% & 0.483 & -4\% & 0.236 & -3\% &0.xxx&-xx\% 
                        & 828.84 & 1.4$\times$ & 687.85 & 1.5$\times$ \\ 
    \cline{2-18}
    DeepTileBars& No Index  & 0.425 && 0.321 && 0.567 && 0.548 && 0.259 & &0.xxx&-xx\%   
                            & 167.20 & & 74.96 &  \\
                & InvIdx    &--&--&--&--&--&--&--&--&--&--&--&--&--&--   \\
                & DeepCT    &--&--&--&--&--&--&--&--&--&--&--&--&--&--   \\
                & SNRM      & 0.356 & -16\% & 0.291 & -9\% & 0.481 & -15\% & 0.434 & -21\% & 0.200 & -23\% &0.xxx&-xx\% 
                            %& 11.47 & 7.3$\times$ & 2.56 & 29.3$\times$ \\
                            & 134.10 & 1.2$\times$ & 58.14 & 1.3$\times$ \\
                & SEINE      & 0.422 & -1\% & 0.322 & 0\% & 0.569 & 0\% & 0.544 & -1\% & 0.255 & -2\% &0.xxx&-xx\% 
                            & 22.62 & 7.4$\times$ & 2.67 & 28.1$\times$ \\
    \bottomrule
\end{tabular*}
\end{table*}
\end{comment}



=======



% for each word $w\in V$ and document $d$ is 


% We standardize the document length to $n_d$, and $t_k$ represents the $k^{th}$ term in a document. 

% To support different level interaction-based NeuIR methods, the corresponding matrices are generated by concatenating the $M_{w, d}$ for each query term $w_i$. 



======



takes the entire document as the smallest interaction unit and generates a scalar value for each w-d pair. 
% It is the same as traditional IR tf-idf based methods, which count the frequency of each term that appears in each document and stored them into inverted index. 
We build our index without segmentation, i.e. 


======

%~\justin{I just clarified this language, is posting list correct terminology?} \grace{yes it is.} 
% For example, if $\sigma_{index}=0$, only the documents containing the corresponding term are stored in the index. 



========



% \subsection{Choice of Segment Size} \label{kernel}

% Our index can support many interaction-based NeurIR methods, only by simply changing the segment size. 
% For segment-level interaction, $M_{w, d} = concat\{\ M(w,S_1),\ M(w,S_2),\ ...\ ,\ M(w,S_{n_b})\ \}, $ where $M(w,S_k)$ is defined by eq (\ref{eq:mat}). 
% Document-level interaction takes the entire document as the smallest interaction unit and generates a scalar value for each w-d pair. 
% It is the same as traditional IR tf-idf based methods, which count the frequency of each term that appears in each document and stored them into inverted index. 
% To support this kind of method, we build our index without segmentation, i.e. the segment size equals the document length. 
% Then the interaction matrix $M_{w, d} = M(w, d)$.
% For term-level interaction, we treat each term as a segment, i.e. the segment size is one term. Similarly, we standardize the document length to $n_d$ here, and $t_k$ represents the $k^{th}$ term in a document.


% At retrieval time, the interaction matrix is $M_{w, d} = concat\{\ M(w,t_1),\ M(w,t_2),\ ...\ ,\ M(w,t_{n_d})\ \}.$ To support different level interaction-based NeuIR methods, the corresponding matrices are generated by concatenating the $M_{w, d}$ for each query term $w_i$. 
% $M_{q,d} = concat\{\ M_{w_1,d},\ M_{w_2,d},\ ...\ ,\ M_{w_q,d}\ \}.$



=======




% ~\justin{start edit to condense normalization details}
% % Suppose the original number of segments in a document is $y$, we resize it into $n_b$. 
% % If $y<n_b$, we pad empty segments behind if the original document is relatively short. 
% % \begin{equation}
% % S_{k}=\left\{  
% % \begin{array}{cc} 
% %     S_k  & k\leq y \\
% %     <empty\ segments> & y<k\leq n_b
% % \end{array} 
% % \right.  
% % \end{equation}
% \justin{end edit}
% \justin{Segmentation applied by textiling should only be used for methods that require it, i.e. not methods that use document-level interaction or term-level interaction. Do any of our methods use anything other than segment level interaction?}
% If $y>n_b$, i.e. the document has more than $n_b$ segments, we squeeze all text after $n_{b-1}^{th}$ segment as the $n_b^{th}$ segment.
% \begin{equation}
% S_{k}=\left\{  
% \begin{array}{cc} 
%     S_k  & k<n_b \\
%     concatenate(S_{n_b}, S_{n_{b+1}},...,S_y) & k=n_b
% \end{array} 
% \right.  
% \end{equation}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.65\linewidth]{graph/index.png}
%   \caption{Structure of SEINE Inverted Index.}
%   %\Description{}
%   \label{fig:index}
% \end{figure}



========



% Different from fixed-size window segmentation, TextTiling revealed the semantic discourse structure and should be more useful for IR tasks.



=========


In order to remove stopwords and balance the indexing time, we 
% 1) count the term frequency of each token 2) sort those tokens descending 3) 
setup thresholds $\sigma_{vocab}^{+}, \sigma_{vocab}^{-} \in [0,1]$ to remove top-$\sigma_{vocab}^+$ and bottom-$\sigma_{vocab}^-$ percent frequent terms from the vocabulary.


==========


% Documents may contain different grammatical forms of a word, such as retrieve, retrieves, and retrieved. 
% There are also families of derivationally related words with similar meanings \cite{cambridge2009online}, such as token, tokenize, and tokenization. 
% These words should play the same role during retrieval, so we use krovetz stemmer \cite{krovetz2000viewing} to chop off the ends of words and remove derivational affixes. 
 
% Besides meaningless tokens and different forms of words, there is also a class of words that may have little value to help match relevant documents given a query, called stopwords.
% A stopword may be identified as a word that has the same likelihood of occurring in those documents not relevant to a query as in those documents relevant to the query \cite{wilbur1992automatic}. 
% There may be two kinds of them: the most common words and the least common words. 
% The most common words are some words like conjunctions, articles, and prepositions, which are functional words that may appear in every document and have no actual meaning.
% The least common words are the ones that have very low frequency in the entire collection. 
% Neither of these words can help differentiate the relevant and irrelevant documents so that they should be removed from the vocabulary.
% On the other hand, since each term in the vocabulary interacts with each document, the indexing time efficiency is a linear function of vocabulary size.



==========


 %and store them in an inverted index.
When queries come in at the retrieval phase, the w-d interactions are looked up from the index and combined into the q-d interaction matrix.
These matrices are then fed into neural ranking models to learn the relevance score.



We can simply look up the w-d interaction for each query term from the pre-computed index and then combine them. 



==========



% \justin{start edit to remove traditional index example}
% % We use the traditional inverted index as an example, in the indexing phase, it counts the frequency of $w$ appearing in $d$, $tf(w,d)$, as the w-d interaction. Each row in the inverted index is a term $w_i$ and its posting list $$PL_i = [d_1: tf(w_i, d_1), d_2: tf(w_i, d_2), ...]$$
% \justin{end edit}


=======

\begin{table*}[htb]
\footnotesize
\caption{Results on MQ2007 and MQ2008. %Improvement (percentage for effectiveness and times for efficiency) of each metric is obtained by comparing to corresponding retrieval method with No Index. 
$^*$ denotes statistically significant degradation on effectiveness and $^\dagger$ for statistically significant improvement on efficiency compared to corresponding retrieval method with No Index.} 
\label{tab:result}
\subtable[\textbf{MQ2007.}]{
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{2}{l}*{6}{lr}*{4}{r}}
\toprule
    \multirow{3}{*}{\bf Indexing} &  \multirow{3}{*}{\bf Retrieval}  &  \multicolumn{12}{c}{\bf Effectiveness}  &  \multicolumn{4}{c}{\bf Efficiency}\\ 
\cline{3-14} \cline{15-18} 
    &  & \multicolumn{2}{c}{P@5}  & \multicolumn{2}{c}{P@10}  & \multicolumn{2}{c}{MAP} & \multicolumn{2}{c}{nDCG@5} & \multicolumn{2}{c}{nDCG@10}  & \multicolumn{2}{c}{Mean nDCG} & \multicolumn{2}{c}{Training (ms)} & \multicolumn{2}{c}{Test (ms)} \\
\cline{2-4} \cline{5-6} \cline{7-8} \cline{9-10} \cline{11-12} \cline{13-14} \cline{15-16} \cline{17-18}       
No Index& Dot Product &0.328&&0.344&&0.418&&0.282&&0.332&&0.418& &&&& \\
        & KNRM  &0.355&&0.382&&0.461&&0.379&&0.412&&0.468&&42.63&&16.70& \\ 
        & HiNT$\diamond$  &0.461&&0.418&&0.505&&0.463&&0.490&&&&1139.34&&1009.11& \\
        & DeepTileBars  &0.429&&0.408&&0.474&&0.398&&0.434&&0.506&&163.91&&73.68& \\
\cline{2-18}
InvIdx$^\ddagger$& BM25$\diamond$    &0.388&&0.366&&0.456&&0.384&&0.414&&&&&&& \\
        % & KNRM    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
        % & HiNT    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
        % & DeepTileBars    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
\cline{2-18}
DeepCT$^\ddagger$ & BM25    &0.315&&0.327&&0.397&&0.266&&0.314&&&&&&&  \\
        % & KNRM    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
        % & HiNT    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
        % & DeepTileBars    &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA& \\
\cline{2-18}
SNRM    & Dot Product   &0.288$^*$&-12\%&0.307$^*$&-11\%&0.368$^*$&-10\%&0.254$^*$&-9\%&0.302$^*$&-9\%&0.378$^*$&-10\%&&&& \\
        & KNRM  &0.322$^*$&-9\%&0.347$^*$&-9\% &0.417$^*$&-10\%&0.337$^*$&-11\%&0.404&-2\% &0.435$^*$&-7\%
                &35.56&1.2$\times$&13.17&1.3$\times$\\
        & HiNT  &0.401$^*$&-13\%&0.358$^*$&-14\%&0.423$^*$&-16\%&0.379$^*$&-18\%&0.402$^*$&-18\%&0.430&
                &958.03&1.2$\times$&860.76&1.1$\times$ \\
        & DeepTileBars  &0.281$^*$&-35\%&0.304$^*$&-25\%&0.359$^*$&-24\%&0.238$^*$&-40\%&0.290$^*$&-33\%&0.365$^*$&-28\%
                        & 131.43 & 1.2$\times$ & 56.97& 1.3$\times$ \\
\cline{2-18}   
SEINE    & Dot Prodect &0.328&0\%&0.344&0\%&0.418&0\%&0.282&0\%&0.332&0\%&0.418&0\%&&&&\\
        & KNRM  &0.342&-4\%&0.372&-2\%&0.447&-3\%&0.374&-1\%&0.401&-3\%&0.462&
                &11.67$^\dagger$&3.7$\times$&1.22$^\dagger$&13.7$\times$ \\
        & HiNT  &0.453&-2\%&0.409&-2\%&0.492&-3\%&0.452&-2\%&0.475&-3\%&0.483&-3\%
                &834.64&1.4$\times$&706.42&1.4$\times$ \\ 
        & DeepTileBars  &0.412&-4\%&0.404&-1\%&0.468&-1\%&0.391&-2\%&0.427&-2\%&0.498&-2\%          &22.62$^\dagger$&7.4$\times$&2.67$^\dagger$&28.1$\times$ \\
\bottomrule
\end{tabular*}
}
\subtable[\textbf{MQ2008.}]{ 
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}*{2}{l}*{6}{lr}*{4}{r}}
\toprule
    \multirow{3}{*}{\bf Indexing} &  \multirow{3}{*}{\bf Retrieval}  &  \multicolumn{12}{c}{\bf Effectiveness}  &  \multicolumn{4}{c}{\bf Efficiency}\\ 
\cline{3-14} \cline{15-18} 
    &  & \multicolumn{2}{c}{P@5}  & \multicolumn{2}{c}{P@10}  & \multicolumn{2}{c}{MAP} & \multicolumn{2}{c}{nDCG@5} & \multicolumn{2}{c}{nDCG@10}  & \multicolumn{2}{c}{Mean nDCG} & \multicolumn{2}{c}{Training (ms)} & \multicolumn{2}{c}{Test (ms)} \\
\cline{2-4} \cline{5-6} \cline{7-8} \cline{9-10} \cline{11-12} \cline{13-14} \cline{15-16} \cline{17-18} 
No Index& Dot Product   &0.333&&0.281&&0.462&&0.411&&0.183&&0.445&&&&&\\
        & KNRM  &0.355&&0.355&&0.472&&0.499&&0.225&&0.463&
                &41.27&&16.86&\\
        & HiNT$\diamond$  &0.367&&0.255&&0.505&&0.501&&0.244&&&     
                &1139.34&&1009.11&\\
        & DeepTileBars  &0.425&&0.321&&0.567&&0.548&&0.259&&0.576&
                        &167.20&&74.96& \\
\cline{2-18}
InvIdx$^\ddagger$  & BM25$\diamond$  &0.337&&0.245&&0.465&&0.461&&0.220&&&&& \\
        % & KNRM  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
        % & HiNT  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
        % & DeepTileBars  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
\cline{2-18}
DeepCT$^\ddagger$  & BM25  &0.307&&0.239&&0.448&&0.400&&0.197&&&&&&&  \\
        % & KNRM  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
        % & HiNT  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
        % & DeepTileBars  &NA&&NA&&NA&&NA&&NA&&NA&&NA&&NA&   \\
\cline{2-18}
SNRM    & Dot Product  &0.380$^\dagger$&14\%&0.300$^\dagger$&7\%&0.513$^\dagger$&11\%&0.483$^\dagger$&18\%&0.223$^\dagger$&22\%&0.513$^\dagger$&15\%&&&& \\
        & KNRM  &0.303$^*$&-15\%&0.229$^*$&-10\%&0.417$^*$&-12\%&0.417$^*$&-16\%&0.199$^*$&-12\%&0.415$^*$&-10\% 
                &36.78&1.1$\times$&12.68&1.3$\times$ \\
        & HiNT  &0.291$^*$&-21\%&0.209$^*$&-18\%&0.401$^*$&-21\%&0.445$^*$&-11\%&0.221$^*$&-10\%&0.436&
                &941.09&1.2$\times$&904.16&1.1$\times$\\
        & DeepTileBars  &0.356$^*$&-16\%&0.291$^*$&-9\%&0.481$^*$&-15\%&0.434$^*$&-21\%&0.200$^*$&-23\%&0.471$^*$&-18\% 
                        &134.10&1.2$\times$&58.14&1.3$\times$ \\
\cline{2-18}
SEINE    & Dot Product   &0.333&0\%&0.281&0\%&0.462&0\%&0.411&0\%&0.183&0\%&0.445&0\%&&&& \\
        & KNRM  &0.346&-3\%&0.252&-1\%&0.462&-2\%&0.485&-3\%&0.218&-3\% &0.445&-4\% 
                &11.58$^\dagger$&3.6$\times$&1.24$^\dagger$&13.6$\times$ \\
        & HiNT  &0.362&-1\%&0.250&-2\%&0.485&-4\%&0.489&-2\%&0.236&-3\%&0.518&
                &828.84&1.4$\times$&687.85&1.5$\times$ \\ 
        & DeepTileBars &0.422&-1\%&0.322&0\%&0.569&0\%&0.544&-1\%&0.255&-2\%&0.573&-1\%
                       &22.62$^\dagger$&7.4$\times$&2.67$^\dagger$&28.1$\times$ \\
\bottomrule
\end{tabular*}
}
\leftline{\tabnote{$^\diamond$ Results reported in Fan et al. \cite{fan2018modeling}. $^\ddagger$ Indexing method is not applicable to KNRM, HiNT, and DeepTileBars.} }
\end{table*} 


================

%aiming to support multiple interaction-based NeurIR retrieval methods.

%Our method  uses flexible interaction units and supports various interaction-based NeurIR methods, by simply modifying a hyper-parameter in our method.

%To facilitate  different NeurIR methods, one can choose the corresponding features, or even update the index by the desired features.



=========



% We observe that the NeurIR methods differ in the interaction units that they use to perform the interaction. The unit can be: 1) Document-level (such as DSSM\cite{huang2013learning}). The entire document is one unit that interacts with each query term or the entire query. 2) Term-level. They include PACRR \cite{hui2017pacrr} and KNRM \cite{xiong2017end}. Each term in the document is treated as a single unit. The interaction matrix of term-level is in the shape of query length by document length. 
% 3) Passage-level or segment-level. They include DeepTileBars \cite{tang2019deeptilebars}, 
% HiNT \cite{fan2018modeling}, and Conv-KNRM \cite{dai2018convolutional}. A document can be segmented by textual discourse units, semantic units, or fixed-size windows. Textual discourse units are usually the natural units of a document such as sentences and paragraphs. Semantic segmentation algorithm such as TextTiling \cite{hearst1994multi} split the document into a sequence of subtopics. Given a large document collection, these interaction matrix can be very big and it takes a long time to be computed. 
\justin{end edit} 
%these methods use a window (or called interaction unit) sliding over the query and every document  and perform calculations within the joint the q window and d window. 


==========


%Hearst proposed TileBar \cite{hearst1995tilebars}, a visualization algorithm that colors each interaction unit based on tf. The more frequent a term occurs in a unit, the darker that unit is. 
%After visualization, the users can better understand the role these relevance signals play during the retrieval.

=========


% Different from the above methods, our index is designed to be query-independent. 


=========


% \grace{Justin: since this is an efficiency paper, I think we should mention and discuss ColBERT. Should also talk about why we do not compare with them in this paper.}



==========


% However, they built an index only for these term representations but not the interaction between terms and documents. When doing retrieval, the document representations were looked up and fed into a deep neural network together with query embedding. 
% This speed up the retrieval time indeed, but it still time-consuming to do interaction between q and d.
% So when applying their index to other NeurIR methods, it will play the role more like a pre-trained word vector model. 


=========


% The reason why a first-stage retriever is necessary is because these methods have deep layers of neural networks and carry heavy computations within their networks, which are time-consuming and computationally-prohibited to work on large document collections and response promptly at query-time. This drawback limits the use of NeurIR methods in real-world applications.


% Ranking is inefficient because it must produce a large query-document interaction matrix in real-time retrieval. 


=========


\subsection{Choice of Segment Size} \label{kernel}

Our index can support many interaction-based NeurIR methods, only by simply changing the segment size. 
For segment-level interaction, $$M_{w, d} = concat\{\ M(w,S_1),\ M(w,S_2),\ ...\ ,\ M(w,S_{n_b})\ \}, $$ where $M(w,S_k)$ is defined by eq (\ref{eq:mat}). 
Document-level interaction takes the entire document as the smallest interaction unit and generates a scalar value for each w-d pair. 
It is the same as traditional IR tf-idf based methods, which count the frequency of each term that appears in each document and stored them into inverted index. 
To support this kind of method, we build our index without segmentation, i.e. the segment size equals the document length. 
Then the interaction matrix $M_{w, d} = M(w, d)$.
For term-level interaction, we treat each term as a segment, i.e. the segment size is one term. Similarly, we standardize the document length to $n_d$ here, and $t_k$ represents the $k^{th}$ term in a document.
So the interaction matrix is $$M_{w, d} = concat\{\ M(w,t_1),\ M(w,t_2),\ ...\ ,\ M(w,t_{n_d})\ \}. $$

To support different level interaction-based NeuIR methods, the corresponding matrices are generated by concatenating the $M_{w, d}$ for each query term $w_i$. 
$$M_{q,d} = concat\{\ M_{w_1,d},\ M_{w_2,d},\ ...\ ,\ M_{w_q,d}\ \}.$$



===========


%\grace{Figure 3 cannot be rectangles. Each should be a square. For all the figures, do not distort them. The fonts inside them should look like very similar to those outside the figures. Do not distort the text.} 
%\grace{In a paper, especially when you are still drafting, do not write out specific counts because you may need to change them later and you will forget about correct them everywhere you wrote them. A trick is to say ``a few", ``a number of ", ``multiple", or just not mention the count. This applies to not-so-essential counts, for instance, here you wrote 3 but your RQs have increased to 4. For counts that are crucial to your methods, you need to be specific and spell it out. } 
%In this section, we discuss multiple research questions (RQ) to better understand the advantages of our proposed indexing method.

%\grace{Also, shall you have the RQs first somewhere in the beginning of the experimental section, and in Results subsection only talk about the answers?} 



========



% This section introduces our proposed segment-based neural indexing method. First, we present the overview of the framework in section \ref{overview}. Then in section \ref{VB}, we introduce the segment-based features.
% In section \ref{SEINE}, we introduced the detailed process of our proposed indexing method. In section \ref{spark} we show how to use the cluster computing tool Spark to accelerate the indexing process. Finally, we discuss how our index can support different NeuIR models by simply changing the segment size in section \ref{kernel}.

========



% This high inefficiency is caused by the high costs of processing the documents and producing a large query-document interaction matrix in real-time retrieval. After receiving a query from the user, these algorithms construct an interaction matrix between the query and words in every document in the collection, and feed it into neural networks to calculate a relevance score. This interaction matrix is usually very big and takes a long time to construct and compute. 

% One class of these models is interaction-based method \citep{guo2016deep, pang2016text, pang2016study, pang2017deeprank, xiong2017end, fan2018modeling, tang2019deeptilebars}. 
% Typically, these methods use a window (or called interaction unit) sliding over the query and document terms and interact the instance in the q windows and d windows to generate the interaction matrix. Then there matrices are fed into neural networks to learn the relevance score.  \grace{merge with the para above}

=========


% Traditional IR methods, such as BM25 \cite{robertson2009probabilistic} and query likelihood \cite{metzler2005markov}, are bag-of-wards models relying on inverted index which stores the relevance signals for each term and document. 
% These signals are frequency-based term weight, such as term frequency (tf), document frequency (df) and inverse document frequency (idf).
% The inverted index is query-independent and built offline, so the traditional IR methods can be applied to web search engines, which handling billions of documents.

% Recent efforts have been devoted to building index for NeurIR models. Zamani et al. proposed SNRM \cite{zamani2018neural} to learn a latent sparse representation for each query and each document. And used that semantic latent term to constructing an inverted index for the whole collection. 
% Dai and Callan proposed DeepCT \cite{dai2019context} that leveraged BERT model to learn context-aware term weights, and these term weights were used as a substitution of tf in the traditional inverted index.
% However, both of their indexes are query-dependent: SNRM trained their network by pairwise models \cite{li2011learning} while DeepCT proposed query term recall as an estimation of the ground truth term importance. 

%\grace{merge the two paras below.}

=============


%In this paper, we propose a novel visualization-based neural indexing method, VBNI, that 

%Our work is a re-design of the NeurIR architecture with the support to building an index for neural models.


%\grace{Here I have a major doubt. Why must we use a 'visualization'-based method? how can 'visualization' directly help with the issues that we mentioned above? I guess we need to express the connection between a few positive points, including 'generalize well to unseen queries', `supporting multiple NeurIR methods', `interaction units with different sizes',  with this `visualization' concept. Call me on slack if you want to discuss.} 


=============


% \grace{the following a few sentences are not transitioned smoothly. When reading them, it feels like you jump among different topics. I guess the beginnings and ends of the sentences are not handled well. It should flow like water.} 
% Their interaction units can be textual discourse units, semantic units, or fixed-size windows. Discourse passages can be  segmented by textual discourse units such as sentences and paragraphs \cite{zamani2018neural} or  by the topics of the text (e.g., TextTiling \cite{hearst1994multi}). 
% DeepTileBars \cite{tang2019deeptilebars} segmented the documents into topical units by TextTiling and produced the interaction matrix by interacted for each segment and the query. 
% HiNT \cite{fan2018modeling} segments the documents by the fixed-size non-overlapping window while Conv-KNRM \cite{dai2018convolutional} by n-gram embedding (fixed-size overlapping window).

==> problem.tex <==
\section{Problem Setup}

%\grace{Add a problem setup section to present what is the mathematically setups for the problem. For instance, what is the input that we are dealing with? What is the input output for the indexing phase and what is for the retrieval phase. Make it mathematically.} 

%\grace{I think the current sections 3 and 4 are dis-organized. You must read all of them and produce new organizations for them. They will probably need new groupings of the content, new subtitles, etc. The key is to have a smooth and correct logic. Right now, it is logically messy.} 

In this section, we describe the ad hoc retrieval task, what are first-stage retrieval and re-ranking, and what are the indexing phase and retrieval phase.

The objective of a ranking task is to retrieve and rank the most relevant documents for a user query, i.e. given a query $q$ and a document corpus $C = \{d_1, d_2, ..., d_{|C|}\}$, we calculate the relevance score for each q-d pair by some functions or neural networks $S_i = f(q, d_i)$.
Then we get a candidate set of N most relevant documents (top-N): $$D_{top-N} = \{d_{P1}..., d_{Pi}, ..., d_{PN}|\forall Pi<Pj, S_{Pi} > S_{Pj}\}.$$

\textbf{First-stage retrieval models} just output the top-N documents for each query. \textbf{Re-ranking models}, or called multi-stage retrieval models, take the $q$ and the corresponding top-N documents $D_{top-N}$ as the inputs of a more complex model (mostly deep neural network), then learn to predict the $S_i = f_{nn}(q, d_i)$ for each q-d pair, and rank these top-N documents again.

The commercial web search engine must process the retrieval fast, especially at first-stage where a query $q$ interacts with tens or hundreds of millions of documents, so the relevance function $f$ must be easy and a small amount of computation. 
An assumption is held that a query is consists of several query terms, and all query terms are in the vocabulary of the corpus. Therefore, we can do term-document (w-d) interaction before we have a query. We call this \textbf{indexing phase} which is query-independent and can be done offline. During the indexing phase, the relevance signal is calculated for each w-d pair and stored as an inverted index.
\textbf{Retrieval phase} is where we generate the q-d interactions. Based on the assumption mentioned before, we can simply look up the w-d interaction for each query term from the pre-computed index and then combine them. Moving these heavy interaction computations ahead and offline greatly improves the efficiency of retrieval.

We use the traditional inverted index as an example, in the indexing phase, it counts the frequency of $w$ appearing in $d$, $tf(w,d)$, as the w-d interaction. Each row in the inverted index is a term $w_i$ and its posting list $$PL_i = [d_1: tf(w_i, d_1), d_2: tf(w_i, d_2), ...]$$
Sometimes we pruning the posting list by removing the item whose $tf=0$. 
In the retrieval phase, we just look up the corresponding tf for each query term from the index and map a simple function as a relevance signal. The summation of them is the relevance score for the q-d pair. 
BM25, a traditional commonly used retrieval algorithm, calculates the relevance score by multiplying terms weights IDF and parameters $k_1$ and $K$. 
$$S_{q,d} = \sum_{w \in q} IDF_w \times \frac{tf(w,d)(k_1+1)}{tf(w,d)+K}$$

NeurIR methods aim to extract more syntactic and semantic features to learn the relevance score. So that the traditional inverted index cannot support them, and there is no index that can support them. 

In this paper, we propose to design a neural index that has more features and can support NeurIR retrieval methods.



==> related_work.tex <==
\section{Related Work}
\sibo{Confirm: SparTerm and SPLADE are using dot product as relevance function. $s(q, d) = q' \cdot d'$, where $q',d'$ are the learned sparse representations}


\sibo{Recent papers added:}

Dense, representation-based retrievers: 
DPR \cite{dpr}, 
SBERT \cite{sbert}, 
ColBert \cite{khattab2020colbert}
RepBERT \cite{repbert}
ANCE (used ANN) \cite{ance}
Condenser \cite{condenser}
RocketQA \cite{rocketqa}


Fast search methods:
FLOPS \cite{flops}, 
SCANN \cite{scann} 
FAISS \cite{faiss}
ANCE \cite{ance}
MIPS \cite{mips}

Sparse, representation-based:
SparTerm \cite{sparterm}, 
SPLADE \cite{splade}, 
SPARTA \cite{sparta}
EPIC \cite{epic}, 
Flops \cite{flops}, 
SNRM \cite{zamani2018neural}

Sparse, interaction-based: 
DeepCT \cite{deepct}
HDCT \cite{hdct} (document retrieval version of DeepCT), 
TILDE \cite{tilde}
KRNM \cite{robertson2009probabilistic}
DeepTileBars \cite{tang2019deeptilebars}). 


%In this section, we discuss related work on NeurIR, indexing and segment-based relevance signal.


% \subsection{Neural Information Retrieval (NeurIR)} 

% NeurIR models use neural networks to rank search results. Due to the complexity of the neural networks, they can not directly use inverted index nor feed the large document corpus as input. 
% So most NeurIR models play a role not truly a retrieval engine but a re-ranker. They first use traditional methods to retrieval a small set of potentially relevant documents and then use deep neural networks to re-rank those documents. 
% %\grace{I move this paragraph here because this is what currently practised at NeurIR. Please add other portion for Area A.}
% NeurIR refers to the application of shallow or deep neural networks to retrieval tasks \cite{mitra2018introduction}. NeurIR models take the raw document and query as input and learn the relevance score for each q-d pair. 
% One class of the NeurIR models is the interaction-based methods \citep{guo2016deep, pang2016text, pang2016study, pang2017deeprank, xiong2017end, fan2018modeling, tang2019deeptilebars}. 
% Typically, these methods use a window (or called interaction unit) sliding over the query and document terms and interact the instance in the q windows and d windows to generate the interaction matrix. Then these matrices are fed into neural networks to learn the relevance score. 
% Mostly we treat the query as a bag of query terms, and the q-d interaction matrix is the combination of the interaction between each query term and each document. 
% So based on the smallest interaction unit for the documents, the interaction-based methods can be further divided into three classes. 1) Document-level (such as \cite{huang2013learning}). The entire document is one unit that interacts with each query term or the entire query. 2) Term-level (such as PACRR \cite{hui2017pacrr} and KNRM \cite{xiong2017end}). Each term in the document is treated as a single unit. The interaction matrix of term-level is in the shape of query length by document length. 3) Passage-level or segment-level. They include DeepTileBars \cite{tang2019deeptilebars}, HiNT \cite{fan2018modeling}, and Conv-KNRM \cite{dai2018convolutional}. A document can be segmented by textual discourse units, semantic units, or fixed-size windows. Textual discourse units are usually the natural units of a document such as sentences and paragraphs. Semantic segmentation algorithm such as TextTiling \cite{hearst1994multi} split the document into a sequence of subtopics. 
% DeepTileBars \cite{tang2019deeptilebars} segmented the documents into topical units by TextTiling and produced the interaction matrix by interacted for each segment and query. 
% HiNT \cite{fan2018modeling} segmented the documents by the fixed-size non-overlapping window while Conv-KNRM \cite{dai2018convolutional} by n-gram embedding (fixed-size overlapping window).

% \subsection{Indexing in IR and NeurIR}

% Traditional IR methods, such as BM25 \cite{robertson2009probabilistic} and query likelihood \cite{metzler2005markov}, are bag-of-wards models relying on inverted index which stores the relevance signals for each term and document. 
% These signals are frequency-based term weight, such as term frequency (tf), document frequency (df) and inverse document frequency (idf).
% The inverted index is query-independent and built offline, so the traditional IR methods can be applied to web search engines, which handling billions of documents.

% Recent efforts have been devoted to building index for NeurIR models. Zamani et al. proposed SNRM \cite{zamani2018neural} to learn a latent sparse representation for each query and each document. And used that semantic latent term to constructing an inverted index for the whole collection. 
% Dai and Callan proposed DeepCT \cite{dai2019context} that leveraged BERT model to learn context-aware term weights, and these term weights were used as a substitution of tf in the traditional inverted index.
% However, both of their indexes are query-dependent: SNRM trained their network by pairwise models \cite{li2011learning} while DeepCT proposed query term recall as an estimation of the ground truth term importance. 

% %\grace{merge the two paras below.}
% MacAvaney et.al \cite{macavaney2020efficient} proposed PreTTR, a transformer to pre-compute term representations at indexing time. They used BERT to train the term representations for each document and stored the compressed embeddings as index.
% However, they built an index only for these term representations but not the interaction between terms and documents. When doing retrieval, the document representations were looked up and fed into a deep neural network together with query embedding. 
% This speeded up the retrieval time indeed, but it still time-consuming to do interaction between q and d.
% So when applying their index to other NeurIR methods, it will play the role more like a pre-trained word vector model.

% Different from the above methods, our index is designed to be query-independent. Based on the assumption that all query terms are in the vocabulary of the corpus, we calculate and store the interaction matrices for each term in the vocabulary and each document.



% \subsection{Segment-Based Relevance}

% In TileBars \cite{hearst1995tilebars}, an algorithm called TextTiling \cite{hearst1994multi} was used to segment the document, which split the document by topic. 
% Then the each query interacted with each segment within a document and the tf based signal was plotted on a two-dimensional grid.
% More frequent a term occurs in a unit, the darker that unit will be. 
% TileBars simultaneously and compactly indicated relative document length, query term frequency, and query term distribution \cite{hearst1995tilebars}.
% It helped users better understand the role these relevance signals play during the retrieval.

% Pang et.al proposed MatchPyramid \cite{pang2016study} for ad-hoc retrieval. They generated term-level interaction matrix and then applied hierarchical convolution to extract matching patterns. They grouped several words together by the kernel size of convolutional layer. 
% Hierarchical matching patterns were learned by a CNN and then fed into a multi-layer perceptron to produce the relevance score between q and d.

% HiNT \cite{fan2018modeling} split each document into segments by fixed-size windows. 
% It extracted both exact matching and semantic matching signals for each q and segment, and further extended the signal to a three-dimensional vector. The three-dimensional vectors were then fed into RNN to learn a relevance score.
% DeepTileBars segmented the documents into a sequence of topical units by TextTiling \cite{hearst1994multi}. 
% It proposed to generate the interaction matrix by three features: tf, inverse document frequency (idf), and word similarity based on the distributional hypothesis \cite{tang2019deeptilebars}. 

% Our method leverage TextTiling, the segmentation algorithm based on topics. We take segments as the smallest interaction unit when building an index. Different from the traditional inverted index whose term-doc interaction value is tf, ours have two kinds of features: term-based features (tf, idf, XOR) and vector-based features calculating word similarity (dot product, cosine similarity).



